PegasusFlow: Parallel Rolling-Denoising Score Sampling for Robot Diffusion Planner Flow Matching

Diffusion models offer powerful generative capabilities for robot trajectory planning, yet their practical deployment on robots is hindered by a critical bottleneck: a reliance on imitation learning from expert demonstrations. This paradigm is often impractical for specialized robots where data is scarce and creates an inefficient, theoretically suboptimal training pipeline. To overcome this, we introduce PegasusFlow, a hierarchical rolling-denoising framework that enables direct and parallel sampling of trajectory score gradients from environmental interaction, completely bypassing the need for expert data. Our core innovation is a novel sampling algorithm, Weighted Basis Function Optimization (WBFO), which leverages spline basis representations to achieve superior sample efficiency and faster convergence compared to traditional methods like MPPI. The framework is embedded within a scalable, asynchronous parallel simulation architecture that supports massively parallel rollouts for efficient data collection. Extensive experiments on trajectory optimization and robotic navigation tasks demonstrate that our approach, particularly Action-Value WBFO (AVWBFO) combined with a reinforcement learning warm-start, significantly outperforms baselines. In a challenging barrier-crossing task, our method achieved a 100% success rate and was 18% faster than the next-best method, validating its effectiveness for complex terrain locomotion planning. https://masteryip.github.io/pegasusflow.github.io/

==> sections/section_3/0notation.tex <==
\begin{table}[t]
    \centering
    \caption{Mathematical Notation}
    \label{tab:notation}
    \begin{tabular}{cl}
        \hline
        \textbf{Symbol}                                       & \textbf{Description}                          \\
        \hline
                                                              & \textbf{Optimal Control}                      \\
        $x \in \mathbb{R}^n$                                  & State vector                                  \\
        $u \in \mathbb{R}^m$                                  & Control input vector                          \\
        $u^*(x,t)$                                            & Optimal control policy                        \\
        $f(\cdot)$                                            & Nonlinear system dynamics function            \\
        $J(\cdot)$                                            & Total cost function                           \\
        $l_f(\cdot)$                                          & Terminal cost function                        \\
        $l(\cdot)$                                            & Cost function                                 \\
        $c_k$                                                 & Command/condition inputs at time $k$          \\
        $o_k$                                                 & Environmental observations at time $k$        \\
        $\alpha$                                              & Exponential discount factor for future costs  \\
        $h$                                                   & Planning horizon                              \\
                                                              & \textbf{MPPI}                                 \\
        $\lambda$                                             & Temperature parameter in MPPI                 \\
        $\sigma$                                              & Noise in sampling                             \\
        $\sigma_k^{(i)}$                                      & Gaussian noise for trajectory $i$ at step $k$ \\
        $\phi(\cdot)$                                         & Kernel function                               \\
        $\boldsymbol{\Sigma}$                                 & Covariance matrix in MPPI update              \\
        $p_0(u)$, $p_1(u)$                                    & Probability distributions in MPPI             \\
                                                              & \textbf{Cubic Spline}                         \\
        $\mathbf{P}$                                          & Matrix of control points                      \\
        $\mathbf{M}$                                          & Cubic spline basis matrix                     \\
        $\mathbf{T}$                                          & Power basis vector                            \\
        $\boldsymbol{u} \in \mathbb{R}^{D \times T}$          & Dense trajectory samples                      \\
        $P_k$                                                 & Control points                                \\
        $\phi_k(t)$                                           & $k$-th basis function                         \\
                                                              & \textbf{WBFO}                                 \\
        $D$                                                   & Trajectory dimension                          \\
        $T, t$                                                & Number of timesteps in trajectory/time index  \\
        $K, k$                                                & Number of nodes/node index                    \\
        $i, j$                                                & Trajectory and node indices                   \\
        $\gamma$                                              & Discount factor in WBFO                       \\
        $r_{i,s}$                                             & Reward of trajectory $i$ at timestep $s$      \\
        $\mathbf{R}_{\text{acc}}(i,t)$                        & Accumulated reward from timestep $t$          \\
        $\mathbf{U} \in \mathbb{R}^{N \times T \times D}$     & Sampled trajectories                          \\
        $\mathbf{R} \in \mathbb{R}^{N \times T}$              & Reward matrix                                 \\
        $\mathbf{R}_{\text{acc}} \in \mathbb{R}^{N \times T}$ & Accumulated reward matrix                     \\
        $\boldsymbol{\Phi} \in \mathbb{R}^{K \times T}$       & Basis function mask matrix                    \\
        $\mathbf{W} \in \mathbb{R}^{N \times K}$              & Weight matrix for trajectories                \\
        $w_{ij}$                                              & Softmax weights for node updates              \\
                                                              & \textbf{Async Simulation}                     \\
        $N$                                                   & Number of sampled trajectories                \\
        $N_m$                                                 & Number of main environments                   \\
        $N_r$                                                 & Number of rollout environments                \\
        $N_{\text{total}}$                                    & Total number of environments                  \\
        \hline
    \end{tabular}
\end{table}
